An Exact Algorithm for Semi-supervised Minimum Sum-of-Squares Clustering

The minimum sum-of-squares clustering (MSSC), or k-means type clustering, is traditionally considered an unsupervised learning task. In recent years, the use of background knowledge to improve the cluster quality and promote interpretability of the clustering process has become a hot research topic at the intersection of mathematical optimization and machine learning research. The problem of taking advantage of background information in data clustering is called semi-supervised or constrained clustering. In this paper, we present a branch-and-cut algorithm for semi-supervised MSSC, where background knowledge is incorporated as pairwise must-link and cannot-link constraints. For the lower bound procedure, we solve the semidefinite programming relaxation of the MSSC discrete optimization model, and we use a cutting-plane procedure for strengthening the bound. For the upper bound, instead, by using integer programming tools, we use an adaptation of the k-means algorithm to the constrained case. For the first time, the proposed global optimization algorithm efficiently manages to solve real-world instances up to 800 data points with different combinations of must-link and cannot-link constraints and with a generic number of features. This problem size is about four times larger than the one of the instances solved by state-of-the-art exact algorithms.

==> tables/glass_7_table.tex <==
\begin{tabular}{cccccccc}
\toprule
     instance &  size &        f &  cp\_iter\_root &  ineq\_root &  gap\_root &  n\_nodes &  time(s) \\
\midrule
 ml\_50\_cl\_0\_0 &   165 &  80.3075 &             4 &       5792 &  0.001166 &        3 &      158 \\
 ml\_50\_cl\_0\_1 &   164 &  88.5778 &             6 &       6460 &  0.000621 &       13 &      397 \\
 ml\_50\_cl\_0\_2 &   164 &  92.1251 &             5 &       6030 &  0.012348 &       59 &      622 \\
 ml\_50\_cl\_0\_3 &   165 &  97.1802 &             8 &       3501 &  0.001637 &       63 &      624 \\
 ml\_50\_cl\_0\_4 &   164 &  92.7342 &            10 &       4418 &  0.002009 &       71 &      746 \\\hline
ml\_25\_cl\_25\_0 &   189 &  77.8657 &            11 &       3253 &  0.003759 &       37 &      677 \\
ml\_25\_cl\_25\_1 &   189 &  76.1155 &             7 &       5940 &  0.000061 &        1 &      139 \\
ml\_25\_cl\_25\_2 &   189 &  74.9960 &            10 &       1712 &  0.000517 &       15 &      434 \\
ml\_25\_cl\_25\_3 &   189 &  70.8828 &            12 &       1508 &  0.001498 &       95 &      872 \\
ml\_25\_cl\_25\_4 &   189 &  79.3567 &            11 &       3406 &  0.001388 &       13 &      374 \\\hline
 ml\_0\_cl\_50\_0 &   214 &  68.1150 &             8 &       6897 &  0.001392 &       13 &      477 \\
 ml\_0\_cl\_50\_1 &   214 &  66.5416 &             8 &       6321 &  0.000590 &        5 &      313 \\
 ml\_0\_cl\_50\_2 &   214 &  68.2079 &            12 &       4029 &  0.000534 &        9 &      444 \\
 ml\_0\_cl\_50\_3 &   214 &  67.5563 &            12 &       2894 &  0.000937 &        5 &      359 \\
 ml\_0\_cl\_50\_4 &   214 &  68.5094 &             8 &       6498 &  0.000132 &        3 &      338 \\\hline
ml\_100\_cl\_0\_0 &   120 &  98.8722 &             5 &       5589 &  0.000123 &        7 &      463 \\
ml\_100\_cl\_0\_1 &   115 & 103.6740 &             6 &       2301 &  0.000279 &        3 &      338 \\
ml\_100\_cl\_0\_2 &   119 & 106.9880 &             2 &       5607 &  0.002563 &        3 &      313 \\
ml\_100\_cl\_0\_3 &   116 & 111.0380 &             5 &       6432 &  0.000063 &        1 &      378 \\
ml\_100\_cl\_0\_4 &   119 & 101.7670 &             7 &       2362 &  0.000341 &       19 &      790 \\\hline
ml\_50\_cl\_50\_0 &   165 &  92.4277 &             7 &       3980 &  0.001138 &       37 &      381 \\
ml\_50\_cl\_50\_1 &   165 &  87.7518 &             6 &       6144 &  0.003818 &       33 &      617 \\
ml\_50\_cl\_50\_2 &   164 &  89.3915 &             8 &       8206 &  0.002587 &       25 &      339 \\
ml\_50\_cl\_50\_3 &   164 &  93.4704 &             7 &       6456 &  0.001442 &       15 &      304 \\
ml\_50\_cl\_50\_4 &   165 &  94.4806 &             9 &       5748 &  0.003127 &       37 &      433 \\\hline
ml\_0\_cl\_100\_0 &   214 &  68.7070 &            10 &       3796 &  0.001144 &       11 &      379 \\
ml\_0\_cl\_100\_1 &   214 &  69.2712 &            10 &       5598 &  0.001668 &       29 &      636 \\
ml\_0\_cl\_100\_2 &   214 &  69.5871 &             6 &       6116 &  0.000977 &        3 &      182 \\
ml\_0\_cl\_100\_3 &   214 &  68.7121 &            11 &       2746 &  0.000622 &        5 &      365 \\
ml\_0\_cl\_100\_4 &   214 &  71.1431 &            12 &       4293 &  0.001665 &        7 &      438 \\
\bottomrule
\end{tabular}


==> tables/global_metrics.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{cccccccccc}
\toprule
      dataset & type &  ari &  ari stdev &  pp ari &  pp ari stdev &  ami &  ami stdev &  pp ami &  pp ami stdev \\
\midrule
         Iris &   ml &     0.891 &      0.064 &        0.874 &         0.057 &     0.886 &      0.055 &        0.871 &         0.047 \\
         Iris &   cl &     0.836 &      0.038 &        0.816 &         0.034 &     0.829 &      0.032 &        0.815 &         0.026 \\
         Iris & mlcl &     0.873 &      0.052 &        0.848 &         0.054 &     0.863 &      0.045 &        0.844 &         0.045 \\
         Wine &   ml &     0.528 &      0.082 &        0.519 &         0.077 &     0.563 &      0.058 &        0.538 &         0.059 \\
         Wine &   cl &     0.429 &      0.028 &        0.409 &         0.032 &     0.454 &      0.023 &        0.436 &         0.034 \\
         Wine & mlcl &     0.491 &      0.071 &        0.457 &         0.056 &     0.512 &      0.052 &        0.484 &         0.042 \\
Connectionist &   ml &     0.065 &      0.040 &        0.051 &         0.048 &     0.056 &      0.033 &        0.037 &         0.034 \\
Connectionist &   cl &     0.077 &      0.074 &        0.056 &         0.057 &     0.061 &      0.055 &        0.041 &         0.042 \\
Connectionist & mlcl &     0.088 &      0.101 &        0.042 &         0.069 &     0.070 &      0.076 &        0.031 &         0.052 \\
        Seeds &   ml &     0.847 &      0.039 &        0.822 &         0.038 &     0.810 &      0.039 &        0.790 &         0.040 \\
        Seeds &   cl &     0.812 &      0.056 &        0.792 &         0.049 &     0.779 &      0.059 &        0.764 &         0.053 \\
        Seeds & mlcl &     0.832 &      0.047 &        0.820 &         0.043 &     0.798 &      0.043 &        0.789 &         0.042 \\
        Glass &   ml &     0.269 &      0.054 &        0.211 &         0.027 &     0.394 &      0.044 &        0.329 &         0.030 \\
        Glass &   cl &     0.205 &      0.013 &        0.169 &         0.010 &     0.322 &      0.016 &        0.290 &         0.023 \\
        Glass & mlcl &     0.223 &      0.014 &        0.195 &         0.020 &     0.345 &      0.019 &        0.320 &         0.019 \\
        Heart &   ml &     0.464 &      0.217 &        0.015 &         0.021 &     0.350 &      0.172 &        0.003 &         0.005 \\
        Heart &   cl &     0.463 &      0.244 &        0.022 &         0.057 &     0.376 &      0.200 &        0.015 &         0.038 \\
        Heart & mlcl &     0.447 &      0.183 &        0.005 &         0.016 &     0.352 &      0.152 &        0.005 &         0.014 \\
    Vertebral &   ml &     0.381 &      0.134 &        0.067 &         0.075 &     0.389 &      0.075 &        0.233 &         0.052 \\
    Vertebral &   cl &     0.375 &      0.091 &        0.273 &         0.066 &     0.345 &      0.082 &        0.279 &         0.054 \\
    Vertebral & mlcl &     0.355 &      0.087 &        0.229 &         0.074 &     0.332 &      0.069 &        0.262 &         0.065 \\
       Accent &   ml &     0.291 &      0.163 &        0.211 &         0.113 &     0.350 &      0.074 &        0.237 &         0.035 \\
       Accent &   cl &     0.057 &      0.006 &        0.028 &         0.019 &     0.203 &      0.015 &        0.180 &         0.009 \\
       Accent & mlcl &     0.071 &      0.033 &        0.064 &         0.015 &     0.234 &      0.019 &        0.192 &         0.014 \\
        Ecoli &   ml &     0.731 &      0.109 &        0.569 &         0.074 &     0.736 &      0.042 &        0.671 &         0.032 \\
        Ecoli &   cl &     0.452 &      0.016 &        0.449 &         0.036 &     0.613 &      0.005 &        0.592 &         0.020 \\
        Ecoli & mlcl &     0.554 &      0.049 &        0.463 &         0.044 &     0.667 &      0.016 &        0.619 &         0.032 \\
      ECG5000 &   ml &     0.611 &      0.085 &        0.582 &         0.053 &     0.603 &      0.033 &        0.576 &         0.025 \\
      ECG5000 &   cl &     0.512 &      0.007 &        0.459 &         0.036 &     0.553 &      0.009 &        0.522 &         0.016 \\
      ECG5000 & mlcl &     0.489 &      0.029 &        0.484 &         0.045 &     0.555 &      0.014 &        0.534 &         0.027 \\
    Computers &   ml &     0.038 &      0.029 &        0.025 &         0.027 &     0.035 &      0.021 &        0.019 &         0.021 \\
    Computers &   cl &     0.041 &      0.025 &        0.013 &         0.018 &     0.037 &      0.018 &        0.010 &         0.013 \\
    Computers & mlcl &     0.035 &      0.011 &        0.015 &         0.017 &     0.032 &      0.007 &        0.011 &         0.013 \\
         Gene &   ml &     0.998 &      0.003 &        0.993 &         0.005 &     0.993 &      0.006 &        0.987 &         0.008 \\
         Gene &   cl &     0.995 &      0.002 &        0.989 &         0.005 &     0.986 &      0.003 &        0.981 &         0.005 \\
         Gene & mlcl &     0.997 &      0.003 &        0.991 &         0.006 &     0.991 &      0.006 &        0.985 &         0.008 \\
\bottomrule
\end{tabular}

\end{table}

==> tables/violated_constraints.tex <==
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
iris & 0 & 50 & 78 & 12.0\% \\
iris & 0 & 50 & 74 & 10.0\% \\
iris & 0 & 50 & 53 & 4.0\% \\
iris & 0 & 50 & 20 & 8.0\% \\
iris & 0 & 50 & 85 & 24.0\% \\
iris & 50 & 0 & 117 & 26.0\% \\
iris & 50 & 0 & 13 & 10.0\% \\
iris & 50 & 0 & 25 & 18.0\% \\
iris & 50 & 0 & 17 & 24.0\% \\
iris & 50 & 0 & 82 & 12.0\% \\
iris & 25 & 25 & 82 & 10.0\% \\
iris & 25 & 25 & 46 & 18.0\% \\
iris & 25 & 25 & 49 & 14.0\% \\
iris & 25 & 25 & 13 & 8.0\% \\
iris & 25 & 25 & 30 & 12.0\% \\
iris & 0 & 100 & 27 & 7.0\% \\
iris & 0 & 100 & 14 & 6.0\% \\
iris & 0 & 100 & 21 & 12.0\% \\
iris & 0 & 100 & 43 & 10.0\% \\
iris & 0 & 100 & 81 & 9.0\% \\
iris & 100 & 0 & 1 & 18.0\% \\
iris & 100 & 0 & 123 & 9.0\% \\
iris & 100 & 0 & 132 & 22.0\% \\
iris & 100 & 0 & 19 & 14.0\% \\
iris & 100 & 0 & 107 & 13.0\% \\
iris & 50 & 50 & 6 & 13.0\% \\
iris & 50 & 50 & 87 & 16.0\% \\
iris & 50 & 50 & 24 & 12.0\% \\
iris & 50 & 50 & 35 & 22.0\% \\
iris & 50 & 50 & 12 & 18.0\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
wine & 0 & 50 & 31 & 12.0\% \\
wine & 0 & 50 & 35 & 20.0\% \\
wine & 0 & 50 & 58 & 16.0\% \\
wine & 0 & 50 & 106 & 24.0\% \\
wine & 0 & 50 & 40 & 22.0\% \\
wine & 50 & 0 & 87 & 38.0\% \\
wine & 50 & 0 & 80 & 36.0\% \\
wine & 50 & 0 & 62 & 44.0\% \\
wine & 50 & 0 & 24 & 38.0\% \\
wine & 50 & 0 & 13 & 42.0\% \\
wine & 25 & 25 & 118 & 28.0\% \\
wine & 25 & 25 & 124 & 28.0\% \\
wine & 25 & 25 & 32 & 42.0\% \\
wine & 25 & 25 & 67 & 26.0\% \\
wine & 25 & 25 & 42 & 38.0\% \\
wine & 0 & 100 & 12 & 24.0\% \\
wine & 0 & 100 & 32 & 24.0\% \\
wine & 0 & 100 & 72 & 20.0\% \\
wine & 0 & 100 & 41 & 23.0\% \\
wine & 0 & 100 & 14 & 18.0\% \\
wine & 100 & 0 & 169 & 37.0\% \\
wine & 100 & 0 & 134 & 46.0\% \\
wine & 100 & 0 & 110 & 43.0\% \\
wine & 100 & 0 & 8 & 41.0\% \\
wine & 100 & 0 & 87 & 44.0\% \\
wine & 50 & 50 & 113 & 29.0\% \\
wine & 50 & 50 & 70 & 30.0\% \\
wine & 50 & 50 & 43 & 26.0\% \\
wine & 50 & 50 & 126 & 42.0\% \\
wine & 50 & 50 & 36 & 38.0\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
connectionist & 0 & 50 & 63 & 50.0\% \\
connectionist & 0 & 50 & 40 & 54.0\% \\
connectionist & 0 & 50 & 43 & 56.0\% \\
connectionist & 0 & 50 & 1 & 48.0\% \\
connectionist & 0 & 50 & 87 & 56.0\% \\
connectionist & 50 & 0 & 117 & 44.0\% \\
connectionist & 50 & 0 & 165 & 46.0\% \\
connectionist & 50 & 0 & 161 & 48.0\% \\
connectionist & 50 & 0 & 27 & 52.0\% \\
connectionist & 50 & 0 & 9 & 42.0\% \\
connectionist & 25 & 25 & 46 & 40.0\% \\
connectionist & 25 & 25 & 27 & 40.0\% \\
connectionist & 25 & 25 & 29 & 44.0\% \\
connectionist & 25 & 25 & 81 & 50.0\% \\
connectionist & 25 & 25 & 47 & 48.0\% \\
connectionist & 0 & 100 & 47 & 54.0\% \\
connectionist & 0 & 100 & 79 & 56.0\% \\
connectionist & 0 & 100 & 72 & 44.0\% \\
connectionist & 0 & 100 & 30 & 51.0\% \\
connectionist & 0 & 100 & 3 & 50.0\% \\
connectionist & 100 & 0 & 103 & 50.0\% \\
connectionist & 100 & 0 & 157 & 45.0\% \\
connectionist & 100 & 0 & 172 & 52.0\% \\
connectionist & 100 & 0 & 24 & 55.0\% \\
connectionist & 100 & 0 & 26 & 69.0\% \\
connectionist & 50 & 50 & 77 & 44.0\% \\
connectionist & 50 & 50 & 26 & 47.0\% \\
connectionist & 50 & 50 & 61 & 55.0\% \\
connectionist & 50 & 50 & 20 & 52.0\% \\
connectionist & 50 & 50 & 41 & 45.0\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
seeds & 0 & 50 & 22 & 14.0\% \\
seeds & 0 & 50 & 107 & 14.0\% \\
seeds & 0 & 50 & 53 & 6.0\% \\
seeds & 0 & 50 & 96 & 8.0\% \\
seeds & 0 & 50 & 66 & 6.0\% \\
seeds & 50 & 0 & 85 & 22.0\% \\
seeds & 50 & 0 & 77 & 14.0\% \\
seeds & 50 & 0 & 161 & 16.0\% \\
seeds & 50 & 0 & 94 & 18.0\% \\
seeds & 50 & 0 & 46 & 20.0\% \\
seeds & 25 & 25 & 29 & 20.0\% \\
seeds & 25 & 25 & 4 & 8.0\% \\
seeds & 25 & 25 & 3 & 26.0\% \\
seeds & 25 & 25 & 57 & 12.0\% \\
seeds & 25 & 25 & 120 & 12.0\% \\
seeds & 0 & 100 & 22 & 11.0\% \\
seeds & 0 & 100 & 49 & 4.0\% \\
seeds & 0 & 100 & 52 & 13.0\% \\
seeds & 0 & 100 & 80 & 14.0\% \\
seeds & 0 & 100 & 62 & 14.0\% \\
seeds & 100 & 0 & 143 & 17.0\% \\
seeds & 100 & 0 & 158 & 17.0\% \\
seeds & 100 & 0 & 2 & 17.0\% \\
seeds & 100 & 0 & 59 & 20.0\% \\
seeds & 100 & 0 & 0 & 22.0\% \\
seeds & 50 & 50 & 101 & 9.0\% \\
seeds & 50 & 50 & 45 & 18.0\% \\
seeds & 50 & 50 & 128 & 19.0\% \\
seeds & 50 & 50 & 33 & 21.0\% \\
seeds & 50 & 50 & 89 & 14.0\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
glass & 0 & 50 & 107 & 26.0\% \\
glass & 0 & 50 & 2 & 16.0\% \\
glass & 0 & 50 & 11 & 26.0\% \\
glass & 0 & 50 & 46 & 26.0\% \\
glass & 0 & 50 & 32 & 28.0\% \\
glass & 50 & 0 & 85 & 62.0\% \\
glass & 50 & 0 & 193 & 54.0\% \\
glass & 50 & 0 & 97 & 56.0\% \\
glass & 50 & 0 & 90 & 62.0\% \\
glass & 50 & 0 & 46 & 70.0\% \\
glass & 25 & 25 & 89 & 34.0\% \\
glass & 25 & 25 & 17 & 38.0\% \\
glass & 25 & 25 & 29 & 52.0\% \\
glass & 25 & 25 & 173 & 26.0\% \\
glass & 25 & 25 & 168 & 46.0\% \\
glass & 0 & 100 & 162 & 25.0\% \\
glass & 0 & 100 & 119 & 26.0\% \\
glass & 0 & 100 & 31 & 22.0\% \\
glass & 0 & 100 & 49 & 19.0\% \\
glass & 0 & 100 & 108 & 27.0\% \\
glass & 100 & 0 & 96 & 53.0\% \\
glass & 100 & 0 & 74 & 52.0\% \\
glass & 100 & 0 & 72 & 59.0\% \\
glass & 100 & 0 & 72 & 63.0\% \\
glass & 100 & 0 & 0 & 54.0\% \\
glass & 50 & 50 & 114 & 40.0\% \\
glass & 50 & 50 & 33 & 38.0\% \\
glass & 50 & 50 & 123 & 50.0\% \\
glass & 50 & 50 & 8 & 39.0\% \\
glass & 50 & 50 & 69 & 42.0\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
heart & 0 & 100 & 114 & 43.0\% \\
heart & 0 & 100 & 41 & 50.0\% \\
heart & 0 & 100 & 7 & 54.0\% \\
heart & 0 & 100 & 50 & 58.0\% \\
heart & 0 & 100 & 167 & 58.0\% \\
heart & 100 & 0 & 92 & 40.0\% \\
heart & 100 & 0 & 67 & 56.0\% \\
heart & 100 & 0 & 114 & 42.0\% \\
heart & 100 & 0 & 10 & 40.0\% \\
heart & 100 & 0 & 155 & 44.0\% \\
heart & 50 & 50 & 30 & 51.0\% \\
heart & 50 & 50 & 18 & 47.0\% \\
heart & 50 & 50 & 194 & 48.0\% \\
heart & 50 & 50 & 195 & 49.0\% \\
heart & 50 & 50 & 126 & 53.0\% \\
heart & 0 & 150 & 0 & 53.3\% \\
heart & 0 & 150 & 22 & 56.7\% \\
heart & 0 & 150 & 8 & 56.0\% \\
heart & 0 & 150 & 65 & 52.0\% \\
heart & 0 & 150 & 16 & 52.0\% \\
heart & 150 & 0 & 270 & 48.7\% \\
heart & 150 & 0 & 130 & 44.7\% \\
heart & 150 & 0 & 56 & 44.7\% \\
heart & 150 & 0 & 136 & 51.3\% \\
heart & 150 & 0 & 112 & 46.0\% \\
heart & 75 & 75 & 53 & 54.0\% \\
heart & 75 & 75 & 15 & 52.7\% \\
heart & 75 & 75 & 186 & 48.7\% \\
heart & 75 & 75 & 220 & 48.7\% \\
heart & 75 & 75 & 93 & 50.7\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
vertebral & 0 & 100 & 43 & 50.0\% \\
vertebral & 0 & 100 & 55 & 47.0\% \\
vertebral & 0 & 100 & 89 & 46.0\% \\
vertebral & 0 & 100 & 197 & 38.0\% \\
vertebral & 0 & 100 & 18 & 42.0\% \\
vertebral & 100 & 0 & 9 & 45.0\% \\
vertebral & 100 & 0 & 13 & 46.0\% \\
vertebral & 100 & 0 & 5 & 38.0\% \\
vertebral & 100 & 0 & 43 & 46.0\% \\
vertebral & 100 & 0 & 215 & 39.0\% \\
vertebral & 50 & 50 & 164 & 36.0\% \\
vertebral & 50 & 50 & 5 & 45.0\% \\
vertebral & 50 & 50 & 171 & 43.0\% \\
vertebral & 50 & 50 & 97 & 45.0\% \\
vertebral & 50 & 50 & 173 & 44.0\% \\
vertebral & 0 & 150 & 55 & 48.7\% \\
vertebral & 0 & 150 & 169 & 53.3\% \\
vertebral & 0 & 150 & 57 & 44.0\% \\
vertebral & 0 & 150 & 163 & 52.7\% \\
vertebral & 0 & 150 & 76 & 44.0\% \\
vertebral & 150 & 0 & 130 & 46.7\% \\
vertebral & 150 & 0 & 33 & 38.0\% \\
vertebral & 150 & 0 & 115 & 38.0\% \\
vertebral & 150 & 0 & 153 & 44.7\% \\
vertebral & 150 & 0 & 77 & 40.7\% \\
vertebral & 75 & 75 & 132 & 49.3\% \\
vertebral & 75 & 75 & 144 & 37.3\% \\
vertebral & 75 & 75 & 95 & 44.0\% \\
vertebral & 75 & 75 & 90 & 52.0\% \\
vertebral & 75 & 75 & 156 & 43.3\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
accent & 0 & 100 & 45 & 19.0\% \\
accent & 0 & 100 & 99 & 27.0\% \\
accent & 0 & 100 & 89 & 17.0\% \\
accent & 0 & 100 & 79 & 19.0\% \\
accent & 0 & 100 & 63 & 16.0\% \\
accent & 100 & 0 & 276 & 73.0\% \\
accent & 100 & 0 & 59 & 81.0\% \\
accent & 100 & 0 & 283 & 75.0\% \\
accent & 100 & 0 & 29 & 77.0\% \\
accent & 100 & 0 & 181 & 78.0\% \\
accent & 50 & 50 & 118 & 46.0\% \\
accent & 50 & 50 & 18 & 48.0\% \\
accent & 50 & 50 & 19 & 51.0\% \\
accent & 50 & 50 & 137 & 43.0\% \\
accent & 50 & 50 & 2 & 42.0\% \\
accent & 0 & 150 & 27 & 25.3\% \\
accent & 0 & 150 & 0 & 14.7\% \\
accent & 0 & 150 & 60 & 18.0\% \\
accent & 0 & 150 & 54 & 14.7\% \\
accent & 0 & 150 & 113 & 18.0\% \\
accent & 150 & 0 & 244 & 83.3\% \\
accent & 150 & 0 & 168 & 76.7\% \\
accent & 150 & 0 & 201 & 72.0\% \\
accent & 150 & 0 & 234 & 76.0\% \\
accent & 150 & 0 & 196 & 75.3\% \\
accent & 75 & 75 & 27 & 44.0\% \\
accent & 75 & 75 & 23 & 42.0\% \\
accent & 75 & 75 & 32 & 45.3\% \\
accent & 75 & 75 & 48 & 50.7\% \\
accent & 75 & 75 & 138 & 50.7\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
ecoli & 0 & 100 & 15 & 0.0\% \\
ecoli & 0 & 100 & 99 & 4.0\% \\
ecoli & 0 & 100 & 194 & 4.0\% \\
ecoli & 0 & 100 & 56 & 4.0\% \\
ecoli & 0 & 100 & 24 & 1.0\% \\
ecoli & 100 & 0 & 2 & 54.0\% \\
ecoli & 100 & 0 & 21 & 57.0\% \\
ecoli & 100 & 0 & 101 & 62.0\% \\
ecoli & 100 & 0 & 15 & 62.0\% \\
ecoli & 100 & 0 & 4 & 59.0\% \\
ecoli & 50 & 50 & 224 & 31.0\% \\
ecoli & 50 & 50 & 76 & 30.0\% \\
ecoli & 50 & 50 & 17 & 41.0\% \\
ecoli & 50 & 50 & 146 & 32.0\% \\
ecoli & 50 & 50 & 111 & 34.0\% \\
ecoli & 0 & 150 & 241 & 7.3\% \\
ecoli & 0 & 150 & 66 & 3.3\% \\
ecoli & 0 & 150 & 17 & 4.7\% \\
ecoli & 0 & 150 & 142 & 2.7\% \\
ecoli & 0 & 150 & 120 & 2.0\% \\
ecoli & 150 & 0 & 10 & 55.3\% \\
ecoli & 150 & 0 & 296 & 56.0\% \\
ecoli & 150 & 0 & 50 & 58.0\% \\
ecoli & 150 & 0 & 7 & 56.7\% \\
ecoli & 150 & 0 & 6 & 60.7\% \\
ecoli & 75 & 75 & 145 & 36.0\% \\
ecoli & 75 & 75 & 217 & 34.7\% \\
ecoli & 75 & 75 & 231 & 24.0\% \\
ecoli & 75 & 75 & 13 & 24.7\% \\
ecoli & 75 & 75 & 67 & 34.7\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
ECG5000 & 0 & 150 & 11 & 2.7\% \\
ECG5000 & 0 & 150 & 15 & 4.7\% \\
ECG5000 & 0 & 150 & 144 & 7.3\% \\
ECG5000 & 0 & 150 & 5 & 6.0\% \\
ECG5000 & 0 & 150 & 65 & 4.7\% \\
ECG5000 & 150 & 0 & 30 & 48.7\% \\
ECG5000 & 150 & 0 & 21 & 50.7\% \\
ECG5000 & 150 & 0 & 102 & 53.3\% \\
ECG5000 & 150 & 0 & 17 & 54.7\% \\
ECG5000 & 150 & 0 & 214 & 47.3\% \\
ECG5000 & 75 & 75 & 235 & 26.7\% \\
ECG5000 & 75 & 75 & 22 & 26.0\% \\
ECG5000 & 75 & 75 & 45 & 34.0\% \\
ECG5000 & 75 & 75 & 113 & 32.0\% \\
ECG5000 & 75 & 75 & 23 & 29.3\% \\
ECG5000 & 0 & 250 & 152 & 6.0\% \\
ECG5000 & 0 & 250 & 69 & 4.4\% \\
ECG5000 & 0 & 250 & 146 & 4.4\% \\
ECG5000 & 0 & 250 & 327 & 6.4\% \\
ECG5000 & 0 & 250 & 171 & 5.6\% \\
ECG5000 & 250 & 0 & 7 & 49.2\% \\
ECG5000 & 250 & 0 & 18 & 47.6\% \\
ECG5000 & 250 & 0 & 317 & 53.6\% \\
ECG5000 & 250 & 0 & 319 & 47.6\% \\
ECG5000 & 250 & 0 & 148 & 48.8\% \\
ECG5000 & 125 & 125 & 286 & 25.6\% \\
ECG5000 & 125 & 125 & 118 & 26.8\% \\
ECG5000 & 125 & 125 & 85 & 26.8\% \\
ECG5000 & 125 & 125 & 261 & 27.6\% \\
ECG5000 & 125 & 125 & 183 & 25.6\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
computers & 0 & 150 & 125 & 48.7\% \\
computers & 0 & 150 & 110 & 50.7\% \\
computers & 0 & 150 & 327 & 51.3\% \\
computers & 0 & 150 & 264 & 50.7\% \\
computers & 0 & 150 & 1 & 58.0\% \\
computers & 150 & 0 & 161 & 40.0\% \\
computers & 150 & 0 & 48 & 44.7\% \\
computers & 150 & 0 & 125 & 53.3\% \\
computers & 150 & 0 & 417 & 48.0\% \\
computers & 150 & 0 & 196 & 58.7\% \\
computers & 75 & 75 & 235 & 39.3\% \\
computers & 75 & 75 & 90 & 47.3\% \\
computers & 75 & 75 & 259 & 47.3\% \\
computers & 75 & 75 & 251 & 52.7\% \\
computers & 75 & 75 & 280 & 50.0\% \\
computers & 0 & 250 & 131 & 55.6\% \\
computers & 0 & 250 & 3 & 47.6\% \\
computers & 0 & 250 & 329 & 54.4\% \\
computers & 0 & 250 & 236 & 52.8\% \\
computers & 0 & 250 & 122 & 52.8\% \\
computers & 250 & 0 & 393 & 44.4\% \\
computers & 250 & 0 & 42 & 48.4\% \\
computers & 250 & 0 & 263 & 40.0\% \\
computers & 250 & 0 & 457 & 48.0\% \\
computers & 250 & 0 & 102 & 44.8\% \\
computers & 125 & 125 & 109 & 52.0\% \\
computers & 125 & 125 & 218 & 48.4\% \\
computers & 125 & 125 & 327 & 53.2\% \\
computers & 125 & 125 & 276 & 55.6\% \\
computers & 125 & 125 & 30 & 46.8\% \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
 dataset & ml &  cl &  seed & violated constraints \\
\midrule
gene & 0 & 200 & 147 & 0.5\% \\
gene & 0 & 200 & 235 & 0.0\% \\
gene & 0 & 200 & 172 & 1.0\% \\
gene & 0 & 200 & 212 & 0.5\% \\
gene & 0 & 200 & 157 & 0.0\% \\
gene & 200 & 0 & 165 & 0.0\% \\
gene & 200 & 0 & 14 & 3.0\% \\
gene & 200 & 0 & 165 & 0.5\% \\
gene & 200 & 0 & 213 & 0.0\% \\
gene & 200 & 0 & 94 & 1.0\% \\
gene & 100 & 100 & 277 & 2.0\% \\
gene & 100 & 100 & 191 & 0.0\% \\
gene & 100 & 100 & 292 & 2.5\% \\
gene & 100 & 100 & 58 & 2.0\% \\
gene & 100 & 100 & 618 & 0.5\% \\
gene & 0 & 400 & 535 & 0.8\% \\
gene & 0 & 400 & 384 & 0.5\% \\
gene & 0 & 400 & 506 & 0.5\% \\
gene & 0 & 400 & 320 & 0.8\% \\
gene & 0 & 400 & 541 & 0.2\% \\
gene & 400 & 0 & 250 & 1.2\% \\
gene & 400 & 0 & 52 & 1.5\% \\
gene & 400 & 0 & 335 & 1.2\% \\
gene & 400 & 0 & 334 & 2.2\% \\
gene & 400 & 0 & 25 & 1.0\% \\
gene & 200 & 200 & 400 & 1.0\% \\
gene & 200 & 200 & 37 & 0.5\% \\
gene & 200 & 200 & 448 & 0.2\% \\
gene & 200 & 200 & 70 & 0.8\% \\
gene & 200 & 200 & 266 & 0.5\% \\

\bottomrule
\end{tabular}
\end{table}

